Predicting Bearings' Degradation Stages for Predictive Maintenance in the Pharmaceutical Industry

In the pharmaceutical industry, the maintenance of production machines must be audited by the regulator. In this context, the problem of predictive maintenance is not when to maintain a machine, but what parts to maintain at a given point in time. The focus shifts from the entire machine to its component parts and prediction becomes a classification problem. In this paper, we focus on rolling-elements bearings and we propose a framework for predicting their degradation stages automatically. Our main contribution is a k-means bearing lifetime segmentation method based on high-frequency bearing vibration signal embedded in a latent low-dimensional subspace using an AutoEncoder. Given high-frequency vibration data, our framework generates a labeled dataset that is used to train a supervised model for bearing degradation stage detection. Our experimental results, based on the FEMTO Bearing dataset, show that our framework is scalable and that it provides reliable and actionable predictions for a range of different bearings.

==> sec1_introduction2.tex <==


%What is the problem?

Rolling-element bearings are a crucial part of manufacturing, 
but strategies to repair (corrective maintenance) or prevent (scheduled maintenance) their degradation are costly. On the one hand, corrective main... leads to machine failure . On the other, scheduled maintenance...


%Why are current solutions not enough?
Predictive maintenance aims to lower the costs by predicting the time of failure and thus choosing the optimal time for maintenance, and can be achieved by a variety of machine learning techniques. Early techniques focus on X, while later techniques with more principled decisions do Y. Unfortunately, all of these suffer from many terrible problems and are not feasible in current manufacturing settings.

%How do we solve it?
We address predictive maintenance three main contributions: (i) a \textbf{domain-knowledge-based approach} for lifetime stage segmentation for a single bearing, (ii) an \textbf{unified model for degradation stage prediction} across bearings, (iii) \textbf{actionable advice for people}. The code is available on \url{https://www.github.com/blabla}



==> sec1_introduction3.tex <==


%Machinery maintenance is a crucial part of manufacturing business. Traditionally companies depending on the cost of machinery and its downtime rely on two main maintenance strategies, namely preventative and corrective maintenance. However, both of these strategies have their significant intrinsic costs. Preventative maintenance is a risk or time-based maintenance scheduling strategy. Maintenance frequency is scheduled based on machinery lifetime estimates provided by its producer or, more often, inferred by statistical risk modeling. As the maintenance is performed regularly despite the condition of the machinery, it results in many discarded healthy parts and wasted human resources maintaining healthy machinery. A way to avoid unnecessary maintenance is to let the machinery run to failure. A corrective, event-based maintenance strategy is easy to implement as it does not require any monitoring, data analysis, or statistical modeling; however, it may result in immense costs. Lack of timely  maintenance is damaging to a machinery due to increased vibrations and overheating which may lead to a secondary damage down the production line or even complete breakdown. What is more, unplanned downtime is expensive as it may be prolonged due to unavailable spare parts or human resources.

Machine learning techniques combined with affordable sensors and processing power gave rise to {\em predictive maintenance} as  means to break the traditional trade-off between machine lifetime maximization (through corrective event-based maintenance) and downtime minimization (through preventive risk-based maintenance) \cite{maintenanceoverview}. With predictive maintenance, interventions on a machine are scheduled based on health condition predictions derived from high frequency data collected by sensors.

Predictive maintenance suffers from a bootstrap problem. Machinery and production processes are costly. Datasets about faulty machinery are small yet expensive to acquire and never shared because of security or competition concerns. As a result, models for predictive maintenance are largely shaped by publicly available datasets obtained running experiments on rolling-element bearings until they fail. A significant body of work leverages such datasets to predict a bearing remaining useful life using regression models. This line of work is hard to validate or tune in production. Worse, predictive maintenance decisions based on remaining time of life predictions can only be based on arbitrary thresholds. How close to failure should maintenance take place?

%An explicit bearing failure point in these dataset led to regression models focused on precise remaining useful life (RUL) prognostics. The issue with RUL models is twofold. First, a complete failure is very unlikely to be observed in the production, leaving industrial applications with no clear target value for model training. Second, RUL models by design put more emphasis on the bearing failure stage and therefore often suffer from late fault detection. This contravene the predictive maintenance goal to use knowledge about actual machinery condition to optimise its operation \cite{pmaintenance}. Early fault detection and degradation process monitoring are essential features of a predictive maintenance model
%that support maintenance professionals in maintenance decision-making. Precise RUL estimation is of a less importance. The key role of a predictive maintenance model is to detect early signs of degradation to provide enough time to react to a developing fault and prevent any secondary damage down the production line.

Instead of modeling bearing degradation as a continuous regression problem, a more interesting approach for predictive maintenance is to classify bearing degradation into discrete stages. This can lead to principled decisions on the timing and type of maintenance based on the predicted degradation stage.

A classification into degradation stages requires labeling sensor measurements. An existing approach is to frame the problem as one class classification \cite{QIU2003127, HONG2014117}. Here the model is trained using only healthy bearing vibration data and the faults are detected when the signal deviates significantly from the healthy signal. Another approach is to train a supervised two class classifier using data from only the beginning of an experiment when a bearing is known to be healthy and the end of the same experiment when the bearing is known to be faulty \cite{s20205846}. While easing up the labeling process these methods however do not provide sufficient bearing fault stage detection granularity.  

The data can also be segmented into multiple stages manually by inspecting plots of vibration signal throughout the whole bearing lifetime in both frequency and time domains \cite{manual, Kimotho2013MachineryPM}, or using clustering algorithms \cite{6798765, 7021915}.

In this paper we build on the aforementioned ideas and present a framework for bearing degradation stage detection. We build on domain knowledge to automate data labeling and use this labeled data to train a supervised classifier for bearing degradation stage detection. This way maintenance professionals get actionable predictions about a bearing condition throughout its lifetime. Robust prediction of early degradation stages is particularly useful for predictive maintenance.

%We use well known machine learning techniques that are easy to implement using existing libraries so that the proposed framework is approachable to maintenance professionals with limited expertise in machine learning. It is, however, worth noting that the framework is also flexible and variety of both labeling and classification step designs can be combined together.


Experimental results show that ...


\textbf{Contributions.} (1) We introduce a framework for bearing degradation stage detection which automatically segments bearing lifetime into degradation stages that are used to train a supervised model for bearing degradation stage detection. (2) We apply domain knowledge and design a k-means bearing lifetime segmentation method based on high-frequency bearing vibration signal embedded in a latent low-dimensional subspace using an AutoEncoder. (3) Our experiments show that...


